ScanQA: 3D Question Answering for Spatial Scene Understanding

We propose a new 3D spatial understanding task of 3D Question Answering (3D-QA). In the 3D-QA task, models receive visual information from the entire 3D scene of the rich RGB-D indoor scan and answer the given textual questions about the 3D scene. Unlike the 2D-question answering of VQA, the conventional 2D-QA models suffer from problems with spatial understanding of object alignment and directions and fail the object identification from the textual questions in 3D-QA. We propose a baseline model for 3D-QA, named ScanQA model, where the model learns a fused descriptor from 3D object proposals and encoded sentence embeddings. This learned descriptor correlates the language expressions with the underlying geometric features of the 3D scan and facilitates the regression of 3D bounding boxes to determine described objects in textual questions and outputs correct answers. We collected human-edited question-answer pairs with free-form answers that are grounded to 3D objects in each 3D scene. Our new ScanQA dataset contains over 40K question-answer pairs from the 800 indoor scenes drawn from the ScanNet dataset. To the best of our knowledge, the proposed 3D-QA task is the first large-scale effort to perform object-grounded question-answering in 3D environments.

==> experiments.tex <==
\begin{table*}[t]
\begin{center}
	\footnotesize\begin{tabular}{lcccccccccc}
        \toprule
Model                & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\
\midrule
\textbf{Valid} \\
W2V NODET 	 &  18.78 & 46.25 & 25.23 & 16.74 & 12.74 & 9.40 & 29.26 & 11.18 & 55.10 & 9.71 \\
VoteNet+MCAN 	 &  17.33 & 45.54 & 28.09 & 16.72 & 10.75 & 6.24 & 29.84 & 11.41 & 54.68 & 10.65 \\
ScanRefer+MCAN (end-to-end) 	 &  18.59 & 46.76 & 26.93 & 16.59 & 11.59 & 7.87 & 30.03 & 11.52 & 55.41 & 11.28 \\
ScanQA 	 &  20.28 & 50.01 & 29.47 & 19.84 & 14.65 & 9.55 & 32.37 & 12.60 & 61.66 & 11.86 \\
\midrule
\textbf{Test w/ objects} \\
W2V NODET 	 &  21.64 & 52.81 & 27.42 & 18.30 & 13.92 & 9.90 & 31.26 & 12.08 & 59.61 & 9.51 \\
VoteNet+MCAN 	 &  19.71 & 50.76 & 29.46 & 17.23 & 10.33 & 6.08 & 30.97 & 12.07 & 58.23 & 10.44 \\
ScanRefer+MCAN (end-to-end) 	 &  20.56 & 52.35 & 27.85 & 17.27 & 11.88 & 7.46 & 30.68 & 11.97 & 57.36 & 10.58 \\
ScanQA 	 &  23.45 & 56.51 & 31.56 & 21.39 & 15.87 & 12.04 & 34.34 & 13.55 & 67.29 & 11.99 \\
\midrule
\textbf{Test w/o objects} \\
W2V NODET 	 &  20.05 & 50.43 & 27.24 & 19.07 & 15.53 & 11.06 & 28.92 & 11.45 & 55.33 & 9.75 \\
VoteNet+MCAN 	 &  18.15 & 48.56 & 29.63 & 17.80 & 11.57 & 7.10 & 29.12 & 11.68 & 53.34 & 10.36 \\
ScanRefer+MCAN (end-to-end) 	 &  19.04 & 49.70 & 26.98 & 16.17 & 11.28 & 7.82 & 28.61 & 11.38 & 53.41 & 10.63 \\
ScanQA 	 &  20.90 & 54.11 & 30.68 & 21.20 & 15.81 & 10.75 & 31.09 & 12.59 & 60.24 & 11.29 \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison for question answering with image captioning metrics.
    }
    %\vspace{-0.5em}
    \label{table:performance2}
\end{center}
%\vspace{-4mm}
\end{table*}

\begin{table*}[t]
\begin{center}
	\footnotesize\begin{tabular}{ccccccccccccc}
        \toprule

%ANSCLS & OBJCLS & LOCAL               & Top-1 EM & Top-10 EM  \\
ANS & OBJ & LOC & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\

\midrule
%\textbf{Test w/ objects} \\
\multicolumn{3}{l}{\textbf{Valid}} \\
\Checkmark &  &  & 10.16 & 36.60 & 11.78 & 5.49 & 0.12 & 0.02 & 16.51 & 6.11 & 26.44 & 4.41 \\
\Checkmark &  \Checkmark & & 14.44 & 43.06 & 19.24 & 13.04 & 10.38 & 0.00 & 23.00 & 8.77 & 42.22 & 6.78 \\
\Checkmark &  & \Checkmark & 16.86 & 45.13 & 22.95 & 15.67 & 12.63 & 9.21 & 26.72 & 10.22 & 49.21 & 8.67 \\
\Checkmark &  \Checkmark & \Checkmark & 20.28 & 50.01 & 29.47 & 19.84 & 14.65 & 9.55 & 32.37 & 12.60 & 61.66 & 11.86 \\
\midrule
%\textbf{Test w/o objects} \\
\multicolumn{3}{l}{\textbf{Test w objects}} \\
\Checkmark &  & & 12.16 & 42.77 & 12.86 & 5.45 & 0.12 & 0.02 & 17.55 & 6.71 & 29.17 & 4.05 \\
\Checkmark &  \Checkmark & & 18.31 & 49.18 & 22.32 & 14.53 & 11.15 & 7.92 & 26.37 & 9.94 & 49.10 & 6.36 \\
\Checkmark &  & \Checkmark &  20.46 & 51.67 & 25.06 & 16.91 & 14.06 & 11.37 & 29.22 & 11.13 & 55.17 & 8.21 \\
\Checkmark & \Checkmark & \Checkmark &  23.45 & 56.51 & 31.56 & 21.39 & 15.87 & 12.04 & 34.34 & 13.55 & 67.29 & 11.99 \\
\midrule
\multicolumn{3}{l}{\textbf{Test w/o objects}} \\
\Checkmark & & & 10.78 & 39.44 & 11.94 & 5.02 & 0.12 & 0.02 & 15.34 & 5.91 & 25.51 & 3.51 \\
\Checkmark &  \Checkmark & & 16.23 & 46.30 & 21.37 & 13.49 & 10.71 & 7.64 & 23.63 & 9.10 & 43.21 & 6.13 \\
\Checkmark &  & \Checkmark &  18.12 & 49.60 & 25.12 & 17.58 & 14.68 & 10.23 & 26.50 & 10.43 & 49.93 & 8.16 \\
\Checkmark & \Checkmark & \Checkmark &  20.90 & 54.11 & 30.68 & 21.20 & 15.81 & 10.75 & 31.09 & 12.59 & 60.24 & 11.29 \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison.
    }
    %\vspace{-0.5em}
    \label{table:performance1}
\end{center}
%\vspace{-4mm}
\end{table*}

\begin{table*}[t]
\begin{center}
	\footnotesize\begin{tabular}{lcccccccccc}
        \toprule
Model                & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\
\midrule
\textbf{valid} \\
ScanQA (xyz)  	 &  20.34 & 49.71 & 29.46 & 19.64 & 13.98 & 9.06 & 32.55 & 12.69 & 62.25 & 12.43 \\
ScanQA (xyz+rgb)  	 &  20.13 & 50.44 & 29.17 & 19.52 & 13.93 & 9.01 & 32.07 & 12.63 & 61.22 & 12.01 \\
ScanQA (xyz+rgb+normal)   	 &  20.00 & 49.11 & 30.00 & 19.25 & 12.91 & 7.47 & 32.54 & 12.55 & 60.83 & 12.45 \\
ScanQA (xyz+multiview)  	 &  20.32 & 50.65 & 30.19 & 19.59 & 14.00 & 9.53 & 32.78 & 12.74 & 62.43 & 12.64 \\
ScanQA (xyz+multiview+normal) 	 &  20.28 & 50.01 & 29.47 & 19.84 & 14.65 & 9.55 & 32.37 & 12.60 & 61.66 & 11.86 \\
\midrule
\textbf{Test w/ objects} \\
ScanQA (xyz)  	 &  24.02 & 55.67 & 32.14 & 21.89 & 16.76 & 12.75 & 34.95 & 13.92 & 68.36 & 11.95 \\
ScanQA (xyz+rgb)  	 &  23.59 & 55.43 & 31.80 & 21.86 & 16.77 & 13.06 & 34.66 & 13.83 & 68.23 & 12.06 \\
ScanQA (xyz+rgb+normal)   	 &  23.49 & 54.50 & 32.11 & 21.87 & 15.92 & 11.29 & 34.40 & 13.67 & 67.94 & 11.72 \\
ScanQA (xyz+multiview)  	 &  23.57 & 55.51 & 32.29 & 21.61 & 16.11 & 12.41 & 34.64 & 13.77 & 67.62 & 12.25 \\
ScanQA (xyz+multiview+normal) 	 &  23.45 & 56.51 & 31.56 & 21.39 & 15.87 & 12.04 & 34.34 & 13.55 & 67.29 & 11.99 \\
\midrule
\textbf{Test w/o objects} \\
ScanQA (xyz)  	 &  20.70 & 53.96 & 31.68 & 22.32 & 17.42 & 12.93 & 31.59 & 12.99 & 61.33 & 12.19 \\
ScanQA (xyz+rgb)  	 &  21.34 & 54.12 & 31.64 & 22.00 & 16.39 & 11.66 & 31.79 & 12.98 & 62.24 & 11.87 \\
ScanQA (xyz+rgb+normal)   	 &  20.90 & 52.72 & 31.48 & 21.28 & 15.76 & 11.04 & 31.56 & 12.84 & 60.73 & 11.66 \\
ScanQA (xyz+multiview)  	 &  21.35 & 53.70 & 31.55 & 21.63 & 15.95 & 11.17 & 31.85 & 12.89 & 61.86 & 11.95 \\
ScanQA (xyz+multiview+normal) 	 &  20.90 & 54.11 & 30.68 & 21.20 & 15.81 & 10.75 & 31.09 & 12.59 & 60.24 & 11.29 \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison.
    }
    %\vspace{-0.5em}
    \label{table:performance2}
\end{center}
%\vspace{-4mm}
\end{table*}



\section{Experiments}
% 導入を書く、モチベーション

%\subsection{Implementation}
\subsection{Experimental Setup}
\noindent \textbf{Data augmentation.} In this experimental setup, we refer to the experimental setup of existing studies on scene understanding of ScanNet~\cite{dai2017scannet}
through languages such as ScanRefer and Scan2Cap~\cite{chen2020scanrefer,chen2021scan2cap}.
We apply data augmentation to our training data and apply rotation about all three axes by a random angle in $[-5\textdegree, 5\textdegree]$and randomly translate the point cloud within 0.5 meters in all directions. Since the ground alignment in ScanNet is incomplete, we rotate it on all axes (not just the top).
% もっとScanReferの設定を参考にしたことを強調した方がいいかも

%\noindent \textbf{Network architecture details.}
%We used VoteNet~\cite{Qi_2019_ICCV} as a backbone for detecting 3D bounding boxes and their features.
%VoteNet used PointNet++~\cite{NIPS2017_d8bf84be} as backbone for 3D feature learning.
%which has four set abstraction (SA) layers and two feature propaga- tion/upsamplng (FP) layers, where the SA layers have in- creasing receptive radius of 0.2, 0.4, 0.8 and 1.2 in meters while they sub-sample the input to 2048, 1024, 512 and 256 points respectively. The two FP layers up-sample the 4th SA layer’s output back to 1024 points with 256-dim fea- tures and 3D coordinates (more details in the appendix).
%The voting layer is realized through a multi-layer per- ceptron with FC output sizes of 256,256,259, where the last FC layer outputs XYZ offset and feature residuals.
%The proposal module is implemented as a set abstraction layer with a post processing MLP2 to generate proposals after the max-pooling. The SA uses radius 0.3 and MLP1 with output sizes of 128, 128, 128. The max-pooled fea- tures are further processed by MLP2 with output sizes of 128,128,5+2NH+4NS+NC wheretheoutputconsists of 2 objectness scores, 3 center regression values, 2NH numbers for heading regression (NH heading bins) and 4NS numbers for box size regression (NS box anchors) and NC numbers for semantic classification.

\noindent \textbf{Training.}
%\subsubsection{Training.}
For training ScanQA model, we used Adam~\cite{kingma2014adam}, batch size $16$, and an initial learning rate of $5\mathrm{e}{-4}$.
We train the model for $30$ epochs and decrease the learning rate by by $0.2$ times after $15$ epochs.
%which is decreased by $0.2$ after $15$ epochs.
%The learning rate is decreased by $5$ after $15$ epochs.
%and then decreased by another 10× after 120 epochs. 
%Training the model to con- vergence on one Volta Quadro GP100 GPU takes around 10 hours on SUN RGB-D and less than 4 hours on ScanNetV2.
%We train the model for $30$ epochs. 
To mitigate fitting exactly against its training data, we set the weight decay factor to $1\mathrm{e}{-5}$.

\noindent \textbf{Evaluation.}
Our ScanQA takes as input both point clouds of the entire scene and a given question and generates object proposals.
For answering a question, our model selects the answer from candidates based on the features of the object proposal corresponding to the question words.
%we back-project multi-view image features to point clouds to leverage the original RGB input
% ↑いまいち。変える
%
%The proposals are post-processed by a 3D NMS module with an IoU threshold of 0.25. 
The goal of our system is to return an accurate answer using 3D-VQA models.
To evaluate QA performance, we used accuracy at 1 and 10 (Acc@1, Acc@10, respectively) as the evaluation metric.
% ↑他の評価指標追加
When using the detection module (VoteNet), we average the results of three evaluation runs with different random seeds.
%We average the results of 3 evaluation runs with different random seeds when using detection module (i.e., VoteNet.)
%We changed the seed and reported the average performance of the three times.
%The evaluation follows the same protocol as in [42] using mean average precision.

\noindent \textbf{Baselines.}
To valid the effects of 3D-VQA model, we prepared several baselines.
%We conducted our empirical investigation using the following models, each of which has different mod- ules. By comparing them, we can ascertain what components determine the generalizations when using 
We conducted our empirical investigation using the following models.

\noindent \textit{\textbf{RandomgImage+2D-VQA}}
%or \noindent \textsf{MCAN + Random} ~\cite{Yu_2019_CVPR}
First, we prepared several 2D-VQA models as baselines to show how our 3D-VQA models outperform 2D-based VQA models for understanding 3D scenes. 
%We used {MCAN} ~\cite{Yu_2019_CVPR} and {Oscar}~\cite{li2020oscar} for 2D-VQA models.
We use {MCAN} ~\cite{Yu_2019_CVPR} for 2D-VQA models.
MCAN is a transformer network~\cite{NIPS2017_3f5ee243} that uses the cross attention mechanism to represent the relationship between question words and features of objects in the image. 
The proposed method uses some of the modules used in mcan, such as self-attention and cross-attention, to create 3D-VQA. By comparing the two, we can confirm the importance of creating a model specialized for 3D-VQA.
%In the end, average the scores of all the responses and choose the most likely answer.
% Large-scalepre-trainingmethodsoflearningcross-modalrep- resentations on image-text pairs 
%Oscar is a BERT-like model trained on a large number of image-text pairs, and has shown high performance not only in VQA, but also in tasks such as image retrieval, image captioning, and natural language visual reasoning.
Since 2D models cannot be directly applied to a 3D environment, images are randomly extracted from the video taken to build the ScanNet dataset. We used a bottom-up attention model~\cite{Anderson_2018_CVPR} for extracting objects' appearance features. Then we applied pre-trained 2D-VQA models to these images and compute the answer score for each image. Finally, we select the most probable answer according to the averaged all answer scores of these images.
%\noindent \textsf{MCAN + Random}

\noindent \textit{\textbf{OracleImage+2D-VQA}}
To investigate the upper bound of the performance of 2D-VQA for questions in 3D space, we used images around target objects associated with question-answer pairs. 
The camera position is set based on the coordinates of the bounding box of the correct object, and the image is captured from the direction and distance that the bounding box reflects the most. Depending on the position of the camera, the object may not be visible, so multiple images were used.
We applied 2D-VQA models to these images similar to RandomImage+2D-VQA.
Note that it is difficult to obtain such images in actual question and answer situations.
By looking at the performance of this method, we can learn the difficulty in solving this 3D-VQA task.

\noindent \textit{\textbf{VoteNet+MCAN}}
VoteNet is a 3D object detection method about locating and recognizing objects in a 3D scene.
This method detect objects in 3D space and extracts their features fed in to the standard VQA model.
Unlike our method,
%it does not take into account object localization and detection for answering questions.
this method does not take into account where the target object is located in the 3D space, what the target object is, etc.
%, such as where the target object is located, or meaning, such as what it is.
% 対象となる物体のローカライゼーション（対象物体が3D空間中のどこにあるか）
% 対象となる物体は何であるか？が考慮されていない。


\noindent \textit{\textbf{ScanRefer+MCAN (pipeline)}}
ScanRefer is a 3D object localization method for localizing a given linguistic description to a corresponding target object in 3D space.
% 内部でVoteNet
ScanRefer internally uses VoteNet to detect objects in the room, and estimates the object corresponding to the description from among the candidate objects.
Even thought ScanRefer cannot be used directly for question answering, we used ScanRefer to identify the object corresponding to the question and applied 2D-VQA (MCAN) to the images around the object localized by ScanRefer.
%3D object localization in RGB-D scans using natural language descriptions. As input, we assume a point cloud of a scanned 3D scene along with a free-form description of a spec- ified target object.
Since both ScanRefer and MCAN are performed separately, it is not possible to learn them end-to-end.

\noindent \textit{\textbf{ScanRefer+MCAN (end-to-end)}}
This method is more sophisticated and closer to the proposed method.
While ScanRefer+MCAN (pipeline) conducts the localization of the object corresponding to the question and question answering separately, in this method, this method learn localization and QA modules simultaneously.
Specifically, the method takes as input the object proposal feature of ScanRefer for VQA models and then 
predict answers based on 3D object features and question content.
Unlike this method, the proposed method shares the same modules for localization and QA and learns the common parts of both simultaneously like multi-task learning~\cite{Zhan_2021_TKDE}.

%We design experiments that leverage the de- tected object information in the input for description gener- ation. Additionally, we show how existing 2D-based cap- tioning methods perform in our newly proposed task.

\subsection{Quantitative Analysis}
%\noindent \textbf{Difficulty of 3D scene VQA.}
% オラクルとの比較で難しさを強調
%Very difficult....
\noindent \textbf{Overall results.} 
We show the 3D-QA performance on ScanQA dataset in Table~\ref{table:performance1} with image captioning metrics.
The best result per column is marked in bold typeface.
We compared our ScanQA with competitive baselines: VoteNet+MCAN, ScanRefer+MCAN (pipeline) and ScanRefer+MCAN (end-to-end).
These baselines share some of the components of the proposed method and can be used to identify which elements are important for 3D-QA.
%We see that ScanRefer+MCAN is  VoteNet+MCAN across most evaluation measures on Test w/ object and Test w/o 
%ScanRefer+MCAN and VoteNet+MCAN are often roughly the same or ScanRefer+MCAN slightly outperforms VoteNet+MCAN.
%suggesting that the object localization module is important to predict 
%correct answer
% 雑（最後？）
The results show that our ScanQA method significantly outperformed all baselines across all data splits over all evaluation metrics. In particular, 
ScanQA significantly outperformed ScanRefer+MCAN (end-to-end), which learns QA and object localization separately over all baselines across all data splits over all evaluation metrics, indicating that ScanQA have succeeded in synergistic learning by sharing object localization and question module.
ScanQA also outperformed VoteNet+MCAN with large margins. This result suggests using localizing objects in 3D space and predicting object categories related questions are important for 3D-QA. We will clarify this point in the ablation study.
Interestingly, VoteNet+MCAN, ScanRefer+MCAN (end-to-end), ScanQA markedly outperformed ScanRefer+MCAN (pipeline), 
which detect target objects related to a question using a pretrained ScanRefer and then apply 2D-QA to surrounding target images indicating that end-to-end training with 3D and language information is important to solve 3D-QA model problems.

%\noindent \textbf{Effect of ...}

\subsection{Ablation Studies}
We conduct an ablation study on our model to examine what components and point cloud features contribute to the 3D-QA performance. Table~\ref{}

\subsection{Qualitative Analysis}

Finally, we demonstrate how multi-step spatiotemporal reasoning works by visualizing ex- amples. Fig. 4 shows some typical examples from the reasoning process of the TS-STMAC network. We selected the frames based on a score, which is the product of the temporal at- tention to a frame and the top five spatial attentions on the regions at each reasoning step. We also show words that receive more attention from the controller unit. The results show the cell tends to identify relevant frames and regions through multi-step reasoning, suggesting that our method effectively incorporated the spatial and temporal features as well as textual information into VideoQA.

==> fig/overview.tex <==
\begin{figure*}
\begin{center}
\includegraphics[width=.99\columnwidth]{example-image-golden}
\hfill
\includegraphics[width=.99\columnwidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Outline -- }
A figure summarizing the entire algorithm
}
\label{fig:overview}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> sec/X_instructions.tex <==
% --- repeat the title (AT: haven't found a more elegant way to do this...)
\twocolumn[
\centering
\Large
\textbf{\LaTeX\ Author Guidelines for \confName~Proceedings (2022)}
\vspace{1.0em}
] %< twocolumn
\appendix

\setcounter{section}{0}
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/abstruct.tex <==

\begin{abstract}
    We propose a new 3D spatial understanding task of 3D Question Answering (3D-QA). In the 3D-QA task, models receive visual information from the entire 3D scene of the rich RGB-D indoor scan and answer the given textual questions about the 3D scene.
    Unlike the 2D-question answering of VQA, the conventional 2D-QA models suffer from problems with spatial understanding of object alignment and directions and fail the object identification from the textual questions in 3D-QA.
    We propose a baseline model for 3D-QA, named ScanQA model, where the model learns a fused descriptor from 3D object proposals and encoded sentence embeddings.
    This learned descriptor correlates the language expressions with the underlying geometric features of the 3D scan and facilitates the regression of 3D bounding boxes to determine described objects in textual questions and outputs correct answers.
    We collected human-edited question-answer pairs with free-form answers that are grounded to 3D objects in each 3D scene. Our new ScanQA dataset contains over 40K question-answer pairs from the 800 indoor scenes drawn from the ScanNet dataset. To the best of our knowledge, the proposed 3D-QA task is the first large-scale effort to perform object-grounded question-answering in 3D environments.
\end{abstract}


==> supp_result/noaug.tex <==
\begin{table*}[t]
\begin{center}
	\footnotesize\begin{tabular}{lcccccccccc}
        \toprule
Model                & EM@1 & EM@10 & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\
\midrule
\textbf{Valid} \\
ScanQA w/o augmentation 	 &  20.60 & 50.35 & 29.24 & 19.14 & 13.87 & 9.16 & 32.43 & 12.60 & 61.91 & 12.09 \\
ScanQA w/ augmentation 	 &  20.28 & 50.01 & 29.47 & 19.84 & 14.65 & 9.55 & 32.37 & 12.60 & 61.66 & 11.86 \\
\midrule
\textbf{Test w/ objects} \\
ScanQA w/o augmentation 	 &  23.45 & 55.69 & 31.48 & 20.86 & 15.62 & 12.36 & 34.49 & 13.56 & 66.61 & 11.45 \\
ScanQA w/ augmentation 	 &  23.45 & 56.51 & 31.56 & 21.39 & 15.87 & 12.04 & 34.34 & 13.55 & 67.29 & 11.99 \\
\midrule
\textbf{Test w/o objects} \\
ScanQA w/o augmentation 	 &  20.90 & 54.24 & 30.69 & 20.84 & 14.77 & 9.58 & 31.15 & 12.57 & 59.82 & 11.38 \\
ScanQA w/ augmentation 	 &  20.90 & 54.11 & 30.68 & 21.20 & 15.81 & 10.75 & 31.09 & 12.59 & 60.24 & 11.29 \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison for the ScanQA model with or without data augmentation
    }
    \label{table:noaug}
    %\vspace{-0.5em}
\end{center}
\vspace{-4mm}
\end{table*}

==> supp_result/result2.tex <==
\begin{table*}[t]
\begin{center}
	\footnotesize\begin{tabular}{lcccccccccc}
        \toprule
%Model                & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\
Model                & EM@1 & EM@10 & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE & METEOR & CIDEr & SPICE \\
\midrule
\textbf{Valid} \\
RandomImage+MCAN & 19.19 & 48.15 & 23.72 & 15.41 & 11.81 & 0.00 & 28.90 & 10.92 & 53.83 & 9.35 \\
OracleImage+MCAN & 22.59 & 49.43 & 26.58 & 18.31 & 15.37 & 8.50 & 33.23 & 12.45 & 63.44 & 12.56\\
VoteNet+MCAN 	 &  17.33 & 45.54 & 28.09 & 16.72 & 10.75 & 6.24 & 29.84 & 11.41 & 54.68 & 10.65 \\
ScanRefer+MCAN (pipeline) & 14.37 & 44.11 & 17.02 & 10.17 & 15.77 & 0.72 & 22.02 & 8.45 & 38.74 & 6.66 \\
ScanRefer+MCAN (e2e) 	 &  18.59 & 46.76 & 26.93 & 16.59 & 11.59 & 7.87 & 30.03 & 11.52 & 55.41 & 11.28 \\
ScanQA 	 &  \textbf{20.28} & \textbf{50.01} & \textbf{29.47} & \textbf{19.84} & \textbf{14.65} & \textbf{9.55} & \textbf{32.37} & \textbf{12.60} & \textbf{61.66} & \textbf{11.86} \\
\midrule
\textbf{Test w/ objects} \\
RandomImage+MCAN  & 22.31 & 53.11 & 26.66 & 18.49 & 16.16 & 14.26 & 31.27 & 12.13 & 60.37 & 9.05\\
OracleImage+MCAN   & 25.34 & 55.93 & 28.70 & 20.11 & 16.78 & 12.89 & 34.59 & 13.42 & 67.24 & 11.93\\
VoteNet+MCAN 	 &  19.71 & 50.76 & 29.46 & 17.23 & 10.33 & 6.08 & 30.97 & 12.07 & 58.23 & 10.44 \\
ScanRefer+MCAN (pipeline) & 17.52 & 49.92 & 19.17 & 10.66 & 0.00 & 0.00 & 24.40 & 9.38 & 44.25 & 6.24 \\
ScanRefer+MCAN (e2e) 	 &  20.56 & 52.35 & 27.85 & 17.27 & 11.88 & 7.46 & 30.68 & 11.97 & 57.36 & 10.58 \\
ScanQA 	 &  \textbf{23.45} & \textbf{56.51} & \textbf{31.56} & \textbf{21.39} & \textbf{15.87} & \textbf{12.04} & \textbf{34.34} & \textbf{13.55} & \textbf{67.29} & \textbf{11.99} \\
\midrule
\textbf{Test w/o objects} \\
RandomImage+MCAN  & 20.82 & 51.23 & 26.29 & 17.90 & 14.27 & 9.66 & 29.23 & 11.54 & 55.64 & 8.87 \\
VoteNet+MCAN 	 &  18.15 & 48.56 & 29.63 & 17.80 & 11.57 & 7.10 & 29.12 & 11.68 & 53.34 & 10.36 \\
ScanRefer+MCAN (pipeline) & 16.47 & 49.05 & 18.71 & 10.98 & 16.53 & 0.76 & 22.45 & 8.76 & 40.81 & 6.41 \\
ScanRefer+MCAN (e2e) 	 &  19.04 & 49.70 & 26.98 & 16.17 & 11.28 & 7.82 & 28.61 & 11.38 & 53.41 & 10.63 \\
ScanQA 	 & \textbf{20.90} & \textbf{54.11} & \textbf{30.68} & \textbf{21.20} & \textbf{15.81} & \textbf{10.75} & \textbf{31.09} & \textbf{12.59} & \textbf{60.24} & \textbf{11.29} \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison for question answering with image captioning metrics. \textbf{e2e} represents an end-to-end model.
    }
    \label{table:performance3D}
    %\vspace{-0.5em}
\end{center}
%\vspace{-4mm}
\end{table*}

\begin{comment}

\begin{table*}[t]
\begin{center}
\footnotesize\begin{tabular}{l|c|cccc|cccc}
\toprule
        & & \multicolumn{4}{c}{PCD} & \multicolumn{4}{c}{Real} \\
Model  & image & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-4 & Top-1 EM & Top-10 EM & BLEU-1 & BLEU-4 \\
\midrule
\textbf{Random Sampling} \\
MCAN & 1 & 16.22 & 47.79 & 16.92 & 0.03 & 17.22 &  49.00 & 18.09 & 0.00 \\
Oscar & 1 & 20.34 & 47.99 & 21.10 & 0.00 & 15.03 & 46.46 & 17.61 &  0.64 \\
MCAN & 3 & 21.74 & 52.41 & 24.86 & 15.19 & 22.31 & 53.11 & 26.66 & 14.26 \\
Oscar & 3  & 20.92 & 49.22 & 23.18 & 0.48 &  22.65 & 52.35 & 24.74 &  0.00  \\
\midrule
\textbf{Oracle} \\
MCAN & 1  & 17.77 & 49.32 & 18.74 & 0.63 & 17.04 & 47.90 & 17.51 & 0.03 \\
Oscar & 1 & 23.89 & 50.92 & 26.14 & 0.00 & 26.73 & 52.21 & 27.63 & 0.58 \\
MCAN & 3 & 23.35 & 53.05 & 25.90 & 10.94 & 25.34 & 55.93 & 28.70 & 12.89 \\
Oscar & 3 & 25.52 & 52.39 & 25.17 & 0.00 & 25.30 & 50.12 & 26.38 & 0.47  \\
\midrule
\multicolumn{2}{l}{\textbf{Other}} \\
\multicolumn{2}{l}{MCAN(top down map)} & 15.76 & 47.15 & 16.53 & 0.00 & - & - & - & - \\
\multicolumn{2}{l}{Oscar(top down map)} & 20.76 & 49.26 & 22.19 & 0.49 & - & - & - & - \\
\multicolumn{2}{l}{ScanRefer+MCAN (pipeline)} & 17.44 & 48.83 & 18.45 & 0.00 & 17.52 & 9.92 & 19.17 & 0.00 \\
\midrule
\midrule
\multicolumn{2}{l}{\textbf{3D-QA}} \\
\multicolumn{2}{l}{ScanQA} &  \textbf{23.45} & \textbf{56.51} & \textbf{31.56} & 12.04  & - & - & - & - \\
\bottomrule
	\end{tabular}
    \caption{
        Performance comparison with 2D image-baselines on test w/ objects. Bold font for the best score among pcd, real image and 3D scan inputs except the oracle results
    }
    \label{table:performance2D}
    %\vspace{-0.5em}
\end{center}
%\vspace{-4mm}
\end{table*}

\end{comment}

% Oscar(pcd, oracle, 3) & 22.27 & 46.59 & 23.01 & 13.96 & 14.23 & 0.00 & 31.37 & 11.53 & 57.98 & 11.11 \\
% Oscar(real, oracle, 3) & 21.39 & 45.05 & 24.29 & 14.19 & 14.21 & 0.67 & 31.24 & 11.33 & 58.23 & 10.51 \\
% 23.45 & 56.51 & 31.56 & 12.04 
